The Aquarius Co-Moving Group is Not a Disrupted Classical Globular Cluster

We present a detailed analysis of high-resolution, high S/N spectra for 5 Aquarius stream stars observed with the MIKE spectrograph on the Magellan Clay telescope. Our sample represents one third of the 15 known members in the stream. We find the stream is not mono-metallic: the metallicity ranges from [Fe/H] = -0.63 to -1.58. No anti-correlation in Na-O abundances is present, and we find a strong positive Mg-Al relationship, similar to that observed in the thick disk. We find no evidence that the stream is a result of a disrupted classical globular cluster, contrary to a previously published claim. High [(Na, Ni, alpha)/Fe] and low [Ba/Y] abundance ratios in the stream suggests it is not a tidal tail from a disrupted dwarf galaxy, either. The stream is chemically indistinguishable from Milky Way field stars with the exception of one candidate, C222531-145437. From its position, velocity, and detailed chemical abundances, C222531-145437 is likely a star that was tidally disrupted from omega-Centauri. We propose the Aquarius stream is Galactic in origin, and could be the result from a disk-satellite perturbation in the Milky Way thick disk on the order of a few Gyr ago: derived orbits, UVW velocities, and angular momenta of the Aquarius members offer qualitative support for our hypothesis. Assuming C222531-145437 is a tidally disrupted member of omega-Centauri, this system is the most likely disk perturber. In the absence of compelling chemical and/or dynamical evidence that the Aquarius stream is the tidal tail of a disrupted satellite, we advocate the "Aquarius group" as a more appropriate description. Like the Canis Major over-density, as well as the Hercules and Monoceros groups, the Aquarius group joins the list of kinematically-identified substructures that are not actually accreted material: they are simply part of the rich complexity of the Milky Way structure.

==> abundances-longtable.tex <==


\begin{longtable*}[t!]{lcrcrrclcrcrrcc}
\caption{\\ Standard Star Abundances\label{tab:standard-star-abundances}} \tabularnewline
\cline{1-13}
Species & $N$ & $\log\epsilon(X)$ & $\sigma$ & [X/H] & [X/Fe] && 
Species & $N$ & $\log\epsilon(X)$ & $\sigma$ & [X/H] & [X/Fe] \tabularnewline 
\cline{1-13} \tabularnewline
% This works.
\endhead
\hline
\multicolumn{13}{r}{Continued..}
\endfoot
\hline
\endlastfoot
\\
\multicolumn{6}{c}{HD\,41667} & \colhead{} & \multicolumn{6}{c}{HD\,44007} \\
\cline{1-6} \cline{8-13}
   C (CH)       &   2 &    6.95 &    0.20 &  --1.48 &  --0.28 && 
   C (CH)       &   2 &    6.66 &    0.20 &  --1.77 &  --0.01 \\ 
   O \textsc{I} &   2 &    7.95 &    0.06 &  --0.74 &    0.46 && 
   O \textsc{I} &   1 &    7.41 &    0.00 &  --1.28 &    0.48 \\ 
  Na \textsc{I} &   3 &    4.90 &    0.18 &  --1.34 &  --0.14 &&
  Na \textsc{I} &   2 &    4.44 &    0.09 &  --1.80 &  --0.04 \\
  Mg \textsc{I} &   4 &    6.72 &    0.10 &  --0.88 &    0.32 &&
  Mg \textsc{I} &   2 &    6.30 &    0.06 &  --1.29 &    0.47 \\
  Al \textsc{I} &   4 &    5.18 &    0.11 &  --1.27 &  --0.07 &&
  Al \textsc{I} &   1 &   :4.80 & \nodata & :--1.65 &   :0.11 \\
  Si \textsc{I} &   5 &    6.55 &    0.06 &  --0.96 &    0.24 &&
  Si \textsc{I} &   5 &    6.07 &    0.07 &  --1.44 &    0.32 \\
   K \textsc{I} &   1 &    4.64 & \nodata &  --0.39 &    0.81 &&
   K \textsc{I} &   1 &    4.31 & \nodata &  --0.72 &    1.04 \\
  Ca \textsc{I} &   4 &    5.47 &    0.06 &  --0.87 &    0.33 &&
  Ca \textsc{I} &   4 &    4.95 &    0.02 &  --1.39 &    0.37 \\
 Sc \textsc{II} &   5 &    2.00 &    0.12 &  --1.15 &    0.05 &&
 Sc \textsc{II} &   5 &    1.32 &    0.12 &  --1.85 &  --0.07 \\
  Ti \textsc{I} &   4 &    3.96 &    0.04 &  --0.99 &    0.21 &&
  Ti \textsc{I} &   1 &    3.48 & \nodata &  --1.47 &    0.29 \\
 Ti \textsc{II} &   3 &    4.09 &    0.25 &  --0.86 &    0.35 &&
 Ti \textsc{II} &   4 &    3.47 &    0.15 &  --1.48 &    0.28 \\
   V \textsc{I} &   4 &    2.85 &    0.11 &  --1.08 &    0.12 &&
   V \textsc{I} &   1 &    2.22 & \nodata &  --1.72 &    0.05 \\
  Cr \textsc{I} &  10 &    4.22 &    0.08 &  --1.42 &  --0.22 &&
  Cr \textsc{I} &  15 &    3.65 &    0.07 &  --1.99 &  --0.22 \\
 Cr \textsc{II} &   2 &    4.54 &    0.05 &  --1.09 &    0.11 &&
 Cr \textsc{II} &   3 &    4.00 &    0.01 &  --1.64 &    0.12 \\
 Mn \textsc{I}  &   3 &    3.87 &    0.04 &  --1.56 &  --0.36 &&
 Mn \textsc{I}  &   2 &    3.21 &    0.06 &  --2.22 &  --0.48 \\
  Fe \textsc{I} &  61 &    6.30 &    0.12 &  --1.20 &    0.00 &&
  Fe \textsc{I} &  51 &    5.74 &    0.13 &  --1.76 &    0.00 \\
 Fe \textsc{II} &  13 &    6.35 &    0.05 &  --1.15 &    0.05 &&
 Fe \textsc{II} &  15 &    5.74 &    0.10 &  --1.76 &  --0.00 \\
  Co \textsc{I} &   3 &    3.73 &    0.06 &  --1.26 &  --0.06 &&
  Co \textsc{I} &   0 & \nodata & \nodata & \nodata & \nodata \\
  Ni \textsc{I} &   7 &    4.94 &    0.12 &  --1.28 &  --0.08 &&
  Ni \textsc{I} &   4 &    4.47 &    0.05 &  --1.75 &    0.01 \\
  Cu \textsc{I} &   1 &    2.29 & \nodata &  --1.90 &  --0.70 &&
  Cu \textsc{I} &   1 &    1.58 & \nodata &  --2.61 &  --0.85 \\
  Zn \textsc{I} &   2 &    3.36 &    0.08 &  --1.20 &    0.00 &&
  Zn \textsc{I} &   2 &    2.83 &    0.05 &  --1.73 &    0.03 \\
  Y \textsc{II} &   5 &    0.97 &    0.19 &  --1.24 &  --0.04 &&
  Y \textsc{II} &   6 &    0.28 &    0.11 &  --1.93 &  --0.16 \\
  Zr \textsc{I} &   2 &    1.42 &    0.05 &  --1.17 &    0.04 &&
  Zr \textsc{I} &   0 & \nodata & \nodata & \nodata & \nodata \\
 Zr \textsc{II} &   1 &    1.28 & \nodata &  --1.30 &  --0.10 &&
 Zr \textsc{II} &   1 &    0.59 & \nodata &  --1.99 &  --0.23 \\
 Ba \textsc{II} &   2 &    0.95 &    0.07 &  --1.23 &  --0.02 &&
 Ba \textsc{II} &   2 &    0.31 &    0.06 &  --1.87 &  --0.11 \\
 La \textsc{II} &   1 &    0.17 & \nodata &  --0.93 &     0.27 &&
 La \textsc{II} &   2 &  --0.57 &    0.05 &  --1.67 &     0.09 \\
 Ce \textsc{II} &   4 &    0.35 &    0.18 &  --1.23 &  --0.02 &&
 Ce \textsc{II} &   3 &  --0.41 &    0.12 &  --1.99 &  --0.23 \\
 Nd \textsc{II} &   9 &    0.54 &    0.10 &  --0.88 &    0.32 &&
 Nd \textsc{II} &   9 &  --0.36 &    0.11 &  --1.78 &  --0.01 \\
 Eu \textsc{II} &   1 &  --0.13 & \nodata &  --0.65 &    0.55 &&
 Eu \textsc{II} &   1 &  --1.16 & \nodata &  --1.68 &    0.08 \\

\cline{1-6} \cline{8-13} \\ \\
\multicolumn{6}{c}{HD\,76932} && \multicolumn{6}{c}{HD\,136316} \\
\cline{1-6} \cline{8-13}
   C (CH)       &   2 &    7.52 &    0.20 &  --0.91 &    0.14 &&
   C (CH)       &   2 &    5.95 &    0.20 &  --2.48 &  --0.50 \\
   O \textsc{I} &   1 &    8.05 & \nodata &  --0.64 &    0.41 &&
   O \textsc{I} &   1 &    7.17 & \nodata &  --1.52 &    0.41 \\
  Na \textsc{I} &   3 &    5.37 &    0.04 &  --0.87 &    0.18 &&
  Na \textsc{I} &   2 &    4.17 &    0.04 &  --2.08 &  --0.14 \\
  Mg \textsc{I} &   3 &    6.95 &    0.20 &  --0.65 &    0.40 &&
  Mg \textsc{I} &   2 &    6.08 &    0.24 &  --1.52 &    0.41 \\
  Al \textsc{I} &   4 &    5.45 &    0.07 &  --1.00 &    0.05 &&
  Al \textsc{I} &   0 & \nodata & \nodata & \nodata & \nodata \\
  Si \textsc{I} &   5 &    6.79 &    0.06 &  --0.72 &    0.33 &&
  Si \textsc{I} &   4 &    5.89 &    0.05 &  --1.62 &    0.31 \\
   K \textsc{I} &   1 &    4.94 & \nodata &  --0.09 &    0.96 &&
   K \textsc{I} &   1 &    3.91 & \nodata &  --1.12 &    0.81 \\
  Ca \textsc{I} &   4 &    5.60 &    0.02 &  --0.74 &    0.31 &&
  Ca \textsc{I} &   4 &    4.71 &    0.02 &  --1.63 &    0.30 \\
 Sc \textsc{II} &   4 &    2.10 &    0.05 &  --1.05 &    0.01 &&
 Sc \textsc{II} &   4 &    1.20 &    0.08 &  --1.95 &  --0.02 \\
  Ti \textsc{I} &   1 &    4.36 & \nodata &  --0.59 &    0.46 &&
  Ti \textsc{I} &   3 &    3.19 &    0.03 &  --1.76 &    0.17 \\
 Ti \textsc{II} &   3 &    4.33 &    0.04 &  --0.62 &    0.44 &&
 Ti \textsc{II} &   3 &    3.44 &    0.10 &  --1.51 &    0.42 \\
   V \textsc{I} &   1 &   :3.33 & \nodata & :--0.60 &   :0.45 &&
   V \textsc{I} &   3 &    1.85 &    0.01 &  --2.08 &  --0.15 \\
  Cr \textsc{I} &  15 &    4.46 &    0.05 &  --1.18 &  --0.13 &&
  Cr \textsc{I} &  12 &    3.49 &    0.05 &  --2.15 &  --0.22 \\
 Cr \textsc{II} &   3 &    4.76 &    0.02 &  --0.88 &    0.17 &&
 Cr \textsc{II} &   2 &    3.90 &    0.02 &  --1.74 &    0.19 \\
  Mn \textsc{I} &   3 &    4.09 &    0.06 &  --1.34 &  --0.28 &&
  Mn \textsc{I} &   3 &    3.09 &    0.03 &  --2.34 &  --0.41 \\
  Fe \textsc{I} &  51 &    6.45 &    0.10 &  --1.05 &    0.00 &&
  Fe \textsc{I} &  62 &    5.57 &    0.11 &  --1.93 &    0.00 \\
 Fe \textsc{II} &  13 &    6.50 &    0.07 &  --1.00 &    0.05 &&
 Fe \textsc{II} &  14 &    5.61 &    0.12 &  --1.89 &    0.04 \\
  Co \textsc{I} &   1 &    3.94 & \nodata &  --1.05 &    0.00 &&
  Co \textsc{I} &   2 &    2.95 &    0.11 &  --1.09 &  --0.11 \\
  Ni \textsc{I} &   5 &    5.29 &    0.02 &  --0.93 &    0.13 &&
  Ni \textsc{I} &   5 &    4.22 &    0.11 &  --2.00 &  --0.07 \\
  Cu \textsc{I} &   1 &    2.53 & \nodata &  --1.66 &  --0.61 &&
  Cu \textsc{I} &   1 &    1.36 & \nodata &  --2.09 &  --0.16 \\
  Zn \textsc{I} &   2 &    3.58 &    0.03 &  --0.98 &    0.07 &&
  Zn \textsc{I} &   2 &    2.72 &    0.03 &  --1.83 &    0.10 \\
  Y \textsc{II} &   5 &    1.14 &    0.05 &  --1.07 &  --0.02 &&
  Y \textsc{II} &   7 &    0.12 &    0.11 &  --2.09 &  --0.16 \\
  Zr \textsc{I} &   0 & \nodata & \nodata & \nodata & \nodata &&
  Zr \textsc{I} &   1 &    0.79 & \nodata &  --1.79 &    0.14 \\
 Zr \textsc{II} &   0 & \nodata & \nodata & \nodata & \nodata &&
 Zr \textsc{II} &   1 &    0.68 & \nodata &  --1.90 &    0.03 \\
 Ba \textsc{II} &   2 &    1.31 &    0.07 &  --0.87 &    0.18 &&
 Ba \textsc{II} &   2 &    0.22 &    0.02 &  --1.96 &  --0.03 \\
 La \textsc{II} &   1 &    0.50 & \nodata &  --0.60 &    0.45 &&
 La \textsc{II} &   1 &  --0.68 & \nodata &  --1.78 &    0.16 \\
 Ce \textsc{II} &   2 &    0.37 &    0.03 &  --1.21 &  --0.16 &&
 Ce \textsc{II} &   5 &  --0.39 &    0.18 &  --1.97 &  --0.04 \\
 Nd \textsc{II} &   3 &    0.56 &    0.06 &  --0.86 &    0.19 &&
 Nd \textsc{II} &  10 &  --0.36 &    0.04 &  --1.78 &    0.15 \\
 Eu \textsc{II} &   1 &  --0.33 & \nodata &  --0.85 &    0.20 &&
 Eu \textsc{II} &   1 &  --1.06 & \nodata &  --1.58 &    0.33 \\

\cline{1-6} \cline{8-13} \\ \\
\multicolumn{6}{c}{HD\,141531} && \multicolumn{6}{c}{HD\,142948} \\
\cline{1-6} \cline{8-13}
   C (CH)       &   2 &    6.33 &    0.20 &  --2.10 &  --0.48 &&
   C (CH)       &   2 &    7.72 &    0.20 &  --0.71 &    0.03 \\
   O \textsc{I} &   2 &    7.33 &    0.01 &  --1.35 &    0.34 &&
   O \textsc{I} &   2 &    8.43 &    0.02 &  --0.26 &    0.47 \\
  Na \textsc{I} &   2 &    4.28 &    0.05 &  --1.96 &  --0.27 &&
  Na \textsc{I} &   3 &    5.73 &    0.13 &  --0.51 &    0.22 \\
  Mg \textsc{I} &   2 &    6.30 &    0.15 &  --1.29 &    0.40 &&
  Mg \textsc{I} &   3 &    7.24 &    0.12 &  --0.36 &    0.38 \\
  Al \textsc{I} &   2 &    4.74 &    0.10 &  --1.71 &  --0.02 &&
  Al \textsc{I} &   4 &    5.94 &    0.08 &  --0.51 &    0.23 \\
  Si \textsc{I} &   5 &    6.03 &    0.10 &  --1.48 &    0.21 &&
  Si \textsc{I} &   5 &    7.07 &    0.05 &  --0.44 &    0.30 \\
   K \textsc{I} &   1 &    3.99 & \nodata &  --1.04 &    0.65 &&
   K \textsc{I} &   1 &    5.04 & \nodata &    0.01 &    0.75 \\
  Ca \textsc{I} &   4 &    4.90 &    0.03 &  --1.44 &    0.25 &&
  Ca \textsc{I} &   4 &    5.78 &    0.01 &  --0.56 &    0.18 \\
 Sc \textsc{II} &   5 &    1.40 &    0.11 &  --1.75 &  --0.06 &&
 Sc \textsc{II} &   5 &    2.57 &    0.12 &  --0.58 &    0.16 \\
  Ti \textsc{I} &   4 &    3.33 &    0.07 &  --1.62 &    0.07 &&
  Ti \textsc{I} &   4 &    4.44 &    0.09 &  --0.51 &    0.23 \\
 Ti \textsc{II} &   4 &    3.71 &    0.08 &  --1.24 &    0.46 &&
 Ti \textsc{II} &   3 &    4.40 &    0.21 &  --0.55 &    0.19 \\
   V \textsc{I} &   4 &    2.10 &    0.07 &  --1.83 &  --0.13 &&
   V \textsc{I} &   5 &    3.31 &    0.04 &  --0.62 &    0.12 \\
  Cr \textsc{I} &  12 &    3.68 &    0.06 &  --1.96 &  --0.27 &&
  Cr \textsc{I} &  13 &    4.67 &    0.15 &  --0.97 &  --0.23 \\
 Cr \textsc{II} &   2 &    4.11 &    0.02 &  --1.53 &    0.16 &&
 Cr \textsc{II} &   3 &    4.88 &    0.03 &  --0.76 &  --0.02 \\
  Mn \textsc{I} &   3 &    3.29 &    0.04 &  --2.14 &  --0.45 &&
  Mn \textsc{I} &   3 &    4.45 &    0.06 &  --0.98 &  --0.24 \\
  Fe \textsc{I} &  54 &    5.81 &    0.06 &  --1.69 &    0.00 &&
  Fe \textsc{I} &  61 &    6.76 &    0.10 &  --0.74 &    0.00 \\
 Fe \textsc{II} &  13 &    5.86 &    0.03 &  --1.64 &    0.05 &&
 Fe \textsc{II} &  13 &    6.75 &    0.06 &  --0.75 &  --0.02 \\
  Co \textsc{I} &   3 &    3.22 &    0.12 &  --1.77 &  --0.08 &&
  Co \textsc{I} &   3 &    4.36 &    0.11 &  --0.63 &  --0.13 \\
  Ni \textsc{I} &   7 &    4.42 &    0.12 &  --1.80 &  --0.11 &&
  Ni \textsc{I} &   5 &    5.62 &    0.04 &  --0.60 &    0.13 \\
  Cu \textsc{I} &   1 &    1.60 & \nodata &  --2.59 &  --0.90 &&
  Cu \textsc{I} &   1 &    3.10 & \nodata &  --1.09 &  --0.35 \\
  Zn \textsc{I} &   2 &    2.80 &    0.04 &  --1.76 &  --0.07 &&
  Zn \textsc{I} &   2 &    3.89 &    0.06 &  --0.67 &    0.07 \\
  Y \textsc{II} &   6 &    0.27 &    0.13 &  --1.94 &  --0.24 &&
  Y \textsc{II} &   6 &    1.33 &    0.32 &  --0.88 &  --0.14 \\
  Zr \textsc{I} &   0 & \nodata & \nodata & \nodata & \nodata &&
  Zr \textsc{I} &   0 & \nodata & \nodata & \nodata & \nodata \\
 Zr \textsc{II} &   1 &    0.75 & \nodata &  --1.83 &  --0.14 &&
 Zr \textsc{II} &   0 & \nodata & \nodata & \nodata & \nodata \\
 Ba \textsc{II} &   2 &    0.39 &    0.05 &  --1.79 &  --0.10 &&
 Ba \textsc{II} &   2 &    1.17 &    0.01 &  --1.01 &  --0.27 \\
 La \textsc{II} &   1 &  --0.56 & \nodata &  --1.67 &    0.03 &&
 La \textsc{II} &   1 &    0.56 & \nodata &  --0.54 &    0.20 \\
 Ce \textsc{II} &   4 &  --0.31 &    0.12 &  --1.89 &  --0.20 &&
 Ce \textsc{II} &   3 &    0.54 &    0.20 &  --1.04 &  --0.30 \\
 Nd \textsc{II} &  10 &  --0.20 &    0.08 &  --1.62 &    0.07 &&
 Nd \textsc{II} &   6 &    0.79 &    0.10 &  --0.63 &    0.11 \\
 Eu \textsc{II} &   1 &  --0.95 & \nodata &  --1.47 &    0.22 &&
 Eu \textsc{II} &   1 &    0.08 & \nodata &  --1.55 &    0.14 \\
\hline
\end{longtable*}



\begin{longtable*}[h!]{lcrcrrclcrcrrcc}
\caption{\\ Program Star Abundances\label{tab:program-star-abundances}} \tabularnewline
\cline{1-13}
Species & $N$ & $\log\epsilon(X)$ & $\sigma$ & [X/H] & [X/Fe] && 
Species & $N$ & $\log\epsilon(X)$ & $\sigma$ & [X/H] & [X/Fe] \tabularnewline 
\cline{1-15} \tabularnewline
% This works.
\endhead
\hline
\multicolumn{13}{r}{Continued..}
\endfoot
\hline
\endlastfoot

\\
\multicolumn{6}{c}{J221821-183424} & \colhead{} & \multicolumn{6}{c}{C222531-145437} \\
\cline{1-6} \cline{8-13}
   C (CH)       &   2 &    6.55 &    0.20 &  --1.88 &  --0.30 &&
   C (CH)       &   2 &    7.15 &    0.20 &  --1.28 &  --0.05 \\
   O \textsc{I} &   2 &    7.55 &    0.04 &  --1.13 &    0.45 &&
   O \textsc{I} &   2 &    7.96 & \nodata &  --0.73 &    0.49 \\
  Na \textsc{I} &   1 &    4.75 & \nodata &  --1.49 &    0.09 &&
  Na \textsc{I} &   2 &    5.12 &    0.02 &  --1.12 &    0.10 \\
  Mg \textsc{I} &   3 &    6.37 &    0.09 &  --1.23 &    0.35 &&
  Mg \textsc{I} &   2 &    6.90 &    0.08 &  --0.70 &    0.53 \\
  Al \textsc{I} &   1 &    5.08 & \nodata &  --1.37 &    0.21 &&
  Al \textsc{I} &   4 &    5.94 &    0.10 &  --0.51 &    0.71 \\
  Si \textsc{I} &   5 &    6.32 &    0.08 &  --1.19 &    0.39 &&
  Si \textsc{I} &   5 &    7.07 &    0.15 &  --0.44 &    0.79 \\
   K \textsc{I} &   1 &    4.34 & \nodata &  --0.69 &    0.89 &&
   K \textsc{I} &   1 &    4.42 & \nodata &  --0.61 &    0.62 \\
  Ca \textsc{I} &   4 &    5.01 &    0.04 &  --1.33 &    0.25 &&
  Ca \textsc{I} &   4 &    5.57 &    0.04 &  --0.77 &    0.45 \\
 Sc \textsc{II} &   4 &    1.50 &    0.12 &  --1.65 &  --0.07 &&
 Sc \textsc{II} &   4 &    2.08 &    0.13 &  --1.07 &    0.16 \\
  Ti \textsc{I} &   0 & \nodata & \nodata & \nodata & \nodata &&
  Ti \textsc{I} &   4 &    4.10 &    0.03 &  --0.85 &    0.37 \\
 Ti \textsc{II} &   4 &    3.80 &    0.13 &  --1.15 &    0.43 &&
 Ti \textsc{II} &   2 &    4.12 &    0.13 &  --0.83 &    0.40 \\
   V \textsc{I} &   3 &    2.28 &    0.01 &  --1.65 &  --0.07 &&
   V \textsc{I} &   5 &    2.91 &    0.10 &  --1.01 &    0.22 \\
  Cr \textsc{I} &  11 &    3.80 &    0.06 &  --1.84 &  --0.26 &&
  Cr \textsc{I} &   8 &    4.24 &    0.17 &  --1.40 &  --0.17 \\
 Cr \textsc{II} &   2 &    4.07 &    0.03 &  --1.57 &    0.01 &&
 Cr \textsc{II} &   1 &    4.38 & \nodata &  --1.26 &  --0.03 \\
  Mn \textsc{I} &   2 &    3.38 &    0.03 &  --2.05 &  --0.46 &&
  Mn \textsc{I} &   3 &    3.98 &    0.05 &  --1.45 &  --0.23 \\
  Fe \textsc{I} &  52 &    5.92 &    0.09 &  --1.58 &    0.00 &&
  Fe \textsc{I} &  60 &    6.27 &    0.10 &  --1.23 &    0.00 \\
 Fe \textsc{II} &  13 &    5.94 &    0.05 &  --1.56 &    0.02 &&
 Fe \textsc{II} &  10 &    6.30 &    0.06 &  --1.20 &    0.03 \\
  Co \textsc{I} &   1 &    3.32 & \nodata &  --1.67 &  --0.09 &&
  Co \textsc{I} &   4 &    3.77 &    0.09 &  --1.22 &    0.00 \\
  Ni \textsc{I} &   5 &    4.61 &    0.14 &  --1.61 &  --0.03 &&
  Ni \textsc{I} &   7 &    5.07 &    0.09 &  --1.15 &    0.08 \\
  Cu \textsc{I} &   1 &    1.81 & \nodata &  --2.38 &  --0.80 &&
  Cu \textsc{I} &   1 &    2.72 & \nodata &  --1.47 &  --0.24 \\
  Zn \textsc{I} &   1 &    3.07 & \nodata &  --1.49 &    0.09 &&
  Zn \textsc{I} &   2 &    3.56 &    0.24 &  --1.00 &    0.23 \\
  Y \textsc{II} &   3 &    0.44 &    0.02 &  --1.77 &  --0.19 &&
  Y \textsc{II} &   5 &    1.78 &    0.16 &  --0.43 &    0.79 \\
  Zr \textsc{I} &   0 & \nodata & \nodata & \nodata & \nodata &&
  Zr \textsc{I} &   3 &    2.07 &    0.05 &  --0.51 &    0.72 \\
 Zr \textsc{II} &   1 &    0.97 & \nodata &  --1.61 &  --0.03 &&
 Zr \textsc{II} &   0 & \nodata & \nodata & \nodata & \nodata \\
 Ba \textsc{II} &   1 &    0.60 & \nodata &  --1.58 &    0.00 &&
 Ba \textsc{II} &   2 &    1.58 &    0.01 &  --0.60 &    0.62 \\
 La \textsc{II} &   1 &  --0.58 & \nodata &  --1.67 &  --0.09 &&
 La \textsc{II} &   2 &    0.51 &    0.02 &  --0.59 &    0.64 \\
 Ce \textsc{II} &   3 &  --0.39 &    0.06 &  --1.97 &  --0.39 &&
 Ce \textsc{II} &   5 &    0.73 &    0.15 &  --0.85 &    0.37 \\
 Nd \textsc{II} &  10 &  --0.22 &    0.07 &  --1.64 &  --0.06 &&
 Nd \textsc{II} &   8 &    0.88 &    0.13 &  --0.54 &    0.69 \\
 Eu \textsc{II} &   1 &  --0.86 &    0.11 &  --1.38 &    0.20 &&
 Eu \textsc{II} &   1 &  --0.29 & \nodata &  --0.81 &    0.42 \\

\cline{1-6} \cline{8-13} \\ \\
\multicolumn{6}{c}{J223504-152834} && \multicolumn{6}{c}{J223811-104126} \\
\cline{1-6} \cline{8-13}
   C (CH)       &   2 &    7.71 &    0.30 &  --0.72 &  --0.10 &&
   C (CH)       &   2 &    7.05 &    0.25 &  --1.38 &    0.05 \\
   O \textsc{I} &   2 &    8.50 &    0.10 &  --0.19 &    0.43 &&
   O \textsc{I}\footnote{Abundance derived from the permitted O \textsc{i} triplet instead of the forbidden [O \textsc{i}] lines, see \S\ref{sec:alpha-elements}} &   3 &    7.41 &    0.13 &  --1.28 &    0.15 \\
  Na \textsc{I} &   3 &    5.87 &    0.12 &  --0.37 &    0.26 &&
  Na \textsc{I} &   1 &    4.89 & \nodata &  --1.35 &    0.08 \\
  Mg \textsc{I} &   3 &    7.48 &    0.15 &  --0.12 &    0.51 &&
  Mg \textsc{I} &   2 &    6.51 &    0.03 &  --1.09 &    0.34 \\
  Al \textsc{I} &   3 &    6.12 &    0.09 &  --0.33 &    0.29 &&
  Al \textsc{I} &   2 &    5.13 &    0.13 &  --1.32 &    0.11 \\
  Si \textsc{I} &   5 &    7.24 &    0.10 &  --0.27 &    0.35 &&
  Si \textsc{I} &   3 &    6.42 &    0.04 &  --1.09 &    0.34 \\
   K \textsc{I} &   1 &    5.05 & \nodata &    0.02 &    0.64 &&
   K \textsc{I} &   1 &    4.50 & \nodata &  --0.53 &    0.90 \\
  Ca \textsc{I} &   4 &    6.06 &    0.03 &  --0.28 &    0.34 &&
  Ca \textsc{I} &   4 &    5.32 &    0.03 &  --1.02 &    0.41 \\
 Sc \textsc{II} &   5 &    2.65 &    0.10 &  --0.50 &    0.13 &&
 Sc \textsc{II} &   2 &    1.60 &    0.03 &  --1.55 &  --0.12 \\
  Ti \textsc{I} &   4 &    4.65 &    0.02 &  --0.30 &    0.32 &&
  Ti \textsc{I} &   0 & \nodata & \nodata & \nodata & \nodata \\
 Ti \textsc{II} &   1 &    4.67 & \nodata &  --0.28 &    0.34 &&
 Ti \textsc{II} &   4 &    3.79 &    0.09 &  --1.16 &    0.27 \\
   V \textsc{I} &   4 &    3.50 &    0.11 &  --0.43 &    0.19 &&
   V \textsc{I} &   1 &    2.45 & \nodata &  --1.48 &  --0.05 \\
  Cr \textsc{I} &   7 &    4.90 &    0.11 &  --0.74 &  --0.11 &&
  Cr \textsc{I} &  12 &    4.10 &    0.06 &  --1.54 &  --0.11 \\
 Cr \textsc{II} &   2 &    4.84 &    0.04 &  --0.79 &  --0.17 &&
 Cr \textsc{II} &   3 &    4.34 &    0.07 &  --1.30 &    0.12 \\
  Mn \textsc{I} &   3 &    4.66 &    0.04 &  --0.77 &  --0.15 &&
  Mn \textsc{I} &   2 &    3.50 &    0.01 &  --1.93 &  --0.51 \\
  Fe \textsc{I} &  63 &    6.88 &    0.12 &  --0.62 &    0.00 &&
  Fe \textsc{I} &  33 &    6.07 &    0.06 &  --1.43 &    0.00 \\
 Fe \textsc{II} &  12 &    6.87 &    0.07 &  --0.63 &  --0.01 &&
 Fe \textsc{II} &   9 &    6.04 &    0.07 &  --1.46 &  --0.03 \\
  Co \textsc{I} &   3 &    4.39 &    0.09 &  --0.60 &    0.02 &&
  Co \textsc{I} &   0 & \nodata & \nodata & \nodata & \nodata \\
  Ni \textsc{I} &   7 &    5.64 &    0.09 &  --0.58 &    0.05 &&
  Ni \textsc{I} &   2 &    4.84 &    0.04 &  --1.38 &    0.05 \\
  Cu \textsc{I} &   1 &    3.72 & \nodata &  --0.47 &    0.15 &&
  Cu \textsc{I} &   1 &    1.96 & \nodata &  --2.23 &  --0.80 \\
  Zn \textsc{I} &   2 &    4.21 &    0.03 &  --0.35 &    0.27 &&
  Zn \textsc{I} &   2 &    3.15 &    0.05 &  --1.41 &    0.02 \\
  Y \textsc{II} &   3 &    1.80 &    0.03 &  --0.41 &    0.21 &&
  Y \textsc{II} &   6 &    0.76 &    0.06 &  --1.45 &  --0.02 \\
  Zr \textsc{I} &   3 &    2.26 &    0.05 &  --0.32 &    0.31 &&
  Zr \textsc{I} &   0 & \nodata & \nodata & \nodata & \nodata \\
 Zr \textsc{II} &   0 & \nodata & \nodata & \nodata & \nodata &&
 Zr \textsc{II} &   0 & \nodata & \nodata & \nodata & \nodata \\
 Ba \textsc{II} &   2 &    1.65 &    0.02 &  --0.53 &    0.10 &&
 Ba \textsc{II} &   2 &    0.78 &    0.07 &  --1.40 &    0.03 \\
 La \textsc{II} &   1 &    0.76 & \nodata &  --0.34 &    0.28 &&
 La \textsc{II} &   0 & \nodata & \nodata & \nodata & \nodata \\
 Ce \textsc{II} &   3 &    0.87 &    0.13 &  --0.71 &  --0.09 &&
 Ce \textsc{II} &   2 &  --0.07 &    0.02 &  --1.65 &  --0.22 \\
 Nd \textsc{II} &   6 &    1.27 &    0.13 &  --0.15 &    0.47 &&
 Nd \textsc{II} &   1 &  --0.25 & \nodata &  --1.67 &  --0.24 \\
 Eu \textsc{II} &   1 &    0.40 & \nodata &  --0.12 &    0.50 &&
 Eu \textsc{II} &   1 &  --0.55 & \nodata &  --1.07 &    0.36 \\

\cline{1-6} \cline{8-13} \\ \\
\multicolumn{7}{c}{C2306265-085103} \\
\cline{1-6}
   C (CH)       &   2 &    7.20 &    0.20 &  --1.23 &  --0.10 \\
   O \textsc{I} &   2 &    8.02 &    0.04 &  --0.67 &    0.46 \\
  Na \textsc{I} &   2 &    5.31 &    0.01 &  --0.93 &    0.21 \\
  Mg \textsc{I} &   2 &    6.90 &    0.06 &  --0.70 &    0.44 \\
  Al \textsc{I} &   4 &    5.65 &    0.08 &  --0.80 &    0.33 \\
  Si \textsc{I} &   5 &    6.78 &    0.08 &  --0.73 &    0.40 \\
   K \textsc{I} &   1 &    4.46 & \nodata &  --0.57 &    0.56 \\
  Ca \textsc{I} &   4 &    5.56 &    0.04 &  --0.78 &    0.35 \\
 Sc \textsc{II} &   3 &    2.15 &    0.09 &  --1.00 &    0.13 \\
  Ti \textsc{I} &   4 &    4.13 &    0.03 &  --0.82 &    0.32 \\
 Ti \textsc{II} &   3 &    4.32 &    0.35 &  --0.63 &    0.51 \\
   V \textsc{I} &   4 &    2.85 &    0.06 &  --1.09 &    0.05 \\
  Cr \textsc{I} &   3 &    4.13 &    0.12 &  --1.51 &  --0.38 \\
 Cr \textsc{II} &   1 &    4.50 & \nodata &  --1.14 &  --0.01 \\
  Mn \textsc{I} &   3 &    4.10 &    0.05 &  --1.33 &  --0.20 \\
  Fe \textsc{I} &  62 &    6.37 &    0.12 &  --1.13 &    0.00 \\
 Fe \textsc{II} &  11 &    6.39 &    0.10 &  --1.11 &    0.02 \\
  Co \textsc{I} &   3 &    3.88 &    0.06 &  --1.11 &    0.02 \\
  Ni \textsc{I} &   7 &    5.11 &    0.07 &  --1.11 &    0.02 \\
  Cu \textsc{I} &   1 &    2.96 & \nodata &  --1.23 &  --0.10 \\
  Zn \textsc{I} &   2 &    3.48 &    0.15 &  --1.08 &    0.05 \\
  Y \textsc{II} &   4 &    1.26 &    0.26 &  --0.95 &    0.18 \\
  Zr \textsc{I} &   3 &    1.60 &    0.05 &  --0.98 &    0.16 \\
 Zr \textsc{II} &   0 & \nodata & \nodata & \nodata & \nodata \\
 Ba \textsc{II} &   2 &    0.95 &    0.10 &  --1.23 &  --0.10 \\
 La \textsc{II} &   1 &    0.07 & \nodata &  --1.03 &    0.10 \\
 Ce \textsc{II} &   2 &    0.09 &    0.02 &  --1.49 &  --0.36 \\
 Nd \textsc{II} &   7 &    0.58 &    0.21 &  --0.84 &    0.29 \\
 Eu \textsc{II} &   1 &  --0.41 & \nodata &  --0.93 &    0.20 \\
 \hline
\end{longtable*}

